How much data is sufficient to learn high-performing algorithms? Generalization guarantees for data-driven algorithm design

Algorithms often have tunable parameters that impact performance metrics such as runtime and solution quality. For many algorithms used in practice, no parameter settings admit meaningful worst-case bounds, so the parameters are made available for the user to tune. Alternatively, parameters may be tuned implicitly within the proof of a worst-case approximation ratio or runtime bound. Worst-case instances, however, may be rare or nonexistent in practice. A growing body of research has demonstrated that data-driven algorithm design can lead to significant improvements in performance. This approach uses a training set of problem instances sampled from an unknown, application-specific distribution and returns a parameter setting with strong average performance on the training set. We provide a broadly applicable theory for deriving generalization guarantees that bound the difference between the algorithm's average performance over the training set and its expected performance. Our results apply no matter how the parameters are tuned, be it via an automated or manual approach. The challenge is that for many types of algorithms, performance is a volatile function of the parameters: slightly perturbing the parameters can cause large changes in behavior. Prior research has proved generalization bounds by employing case-by-case analyses of greedy algorithms, clustering algorithms, integer programming algorithms, and selling mechanisms. We uncover a unifying structure which we use to prove extremely general guarantees, yet we recover the bounds from prior research. Our guarantees apply whenever an algorithm's performance is a piecewise-constant, -linear, or -- more generally -- piecewise-structured function of its parameters. Our theory also implies novel bounds for voting mechanisms and dynamic programming algorithms from computational biology.

==> experiments_intro.tex <==
In this section, we provide experiments demonstrating the utility of our theoretical bounds. We highlight two key observations that these simulations illustrate.
\begin{observation}\label{obs:estimate}
	In the context of sequence alignment (Appendix~\ref{app:sequence}), we demonstrate that an algorithm's performance on average over a training set with finite size provides a tight estimate of its expected performance on the underlying distribution. This fast convergence mirrors the theoretical guarantees in this paper.
	\end{observation}

\begin{observation}\label{obs:two_families}
\textnormal{We show that two algorithms for the same computational problem may require markedly different training set sizes to avoid overfitting. We demonstrate this---using a real data set---in the context of selling mechanism design for revenue maximization (Appendix~\ref{app:experiments_revenue}) and voting mechanism design for social welfare maximization (Appendix~\ref{app:experiments_welfare}). In each of these domains, we analyze two algorithm families that have surface-level similarities, but we empirically illustrate that one family requires more samples to avoid overfitting than the other. Therefore, it is crucial to calculate a family's pseudo-dimension to provide accurate guarantees. This paper provides tools for doing so.}
	\end{observation} 
